Taxes Are All You Need: Integration of Taxonomical Hierarchy Relationships into the Contrastive Loss

In this work, we propose a novel supervised contrastive loss that enables the integration of taxonomic hierarchy information during the representation learning process. A supervised contrastive loss operates by enforcing that images with the same class label (positive samples) project closer to each other than images with differing class labels (negative samples). The advantage of this approach is that it directly penalizes the structure of the representation space itself. This enables greater flexibility with respect to encoding semantic concepts. However, the standard supervised contrastive loss only enforces semantic structure based on the downstream task (i.e. the class label). In reality, the class label is only one level of a \emph{hierarchy of different semantic relationships known as a taxonomy}. For example, the class label is oftentimes the species of an animal, but between different classes there are higher order relationships such as all animals with wings being ``birds". We show that by explicitly accounting for these relationships with a weighting penalty in the contrastive loss we can out-perform the supervised contrastive loss. Additionally, we demonstrate the adaptability of the notion of a taxonomy by integrating our loss into medical and noise-based settings that show performance improvements by as much as 7%.

==> Sections/abstract.tex <==
In this work, we propose a new framework for hard contrastive learning based on decomposing the negative distribution into informed subsets. Hardness-aware contrastive learning argues that certain negative samples in a batch are more informative due to sharing semantic features in common with the anchor image. Integrating hardness into contrastive learning frameworks involves computing a weighting distribution over the set of negatives where harder negatives contribute more to the overall loss. The main limitation of existing works is that this hardness distribution is computed as a function of the entire batch of negatives, rather than explicitly identifying the hardest negatives with respect to each image. To address this, we propose to first decompose the negative distribution into what we define as hard and regular subsets specific to each anchor image based on thresholding pairwise cosine similarity values with the anchor embedding. The hard negative weighting distribution is then computed with respect to this instance-specific hard subset, rather than the batch as a whole. We theoretically show that this decomposition of hardness is motivated by multiple importance sampling and semantically interpret this hardness based on superclasses. Additionally, we introduce the idea of domain-specific hardness and show how the adaptability of our framework enables integrating hard negatives based on application-specific data structures. We empirically validate this approach across  5 different datasets, 3 training settings, and in comparison with 7 state-of-the-art contrastive learning algorithms. This includes a 4\% accuracy improvement over a previous hardness strategy and 2\% improvement over baseline NNCLR.

==> Sections/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}

In this work, we introduce a new hard contrastive learning framework that alleviates the limitations of previous hardness weighting distributions. Namely, we show how decomposing the distribution of negatives via a cosine similarity and superclass thresholding can effectively result in a set of negatives that better approximates the hardness distribution. We show how this relates to concepts related to multiple MC importance sampling. Additionally, we show that this strategy works in optimally configured contrastive learning training settings, across a variety of datasets, and in comparison with state of the art approaches when integrated appropriately. All of these advantages exist without requiring expensive computations over previous hardness methods. We also show through our supervised experiments that the notion of hardness can be generalized in such a way that it can be adapted to the domain of interest. 

==> Sections/introduction.tex <==
\section{Introduction}



Contrastive learning \cite{le2020contrastive} refers to a family of self-supervision strategies that build an embedding space where similar pairs of images (positives) project closer together and dissimilar pairs of images (negatives) project apart. In \cite{chen2020simple}, positive pairs are generated through an augmentation of an anchor image and all other instances in a batch are the negative set. While this setup has shown great empirical success and has motivated other works \cite{dwibedi2021little,chen2020improved}, the simple batch assignment of negatives 
 does not consider the hardness relationship that exists with respect to the anchor image. We define hardness as a distribution across the negative set that represents how semantically similar each negative instance is to the anchor image.   For example, in the batch presented in Figure \ref{fig: batch_view}, we observe that, with respect to the anchor image of a flamingo, the spoonbill negative has more semantic structures in common compared to that of the rest of the batch. Intuitively, this means that it is more difficult to contrast between the two and thus the model is forced to learn more specific features of the flamingo class in order to effectively distinguish it from the closely related spoonbill~\cite{9190927, alregib2022explanatory}. Thus, this harder negative is more informative in identifying distinguishing features of the anchor image and should contribute more to the overall loss.
 
% Ideally this means that the resulting contrastive loss should weight these samples as more important, but approximating this hardness distribution is not trivial in practice.

\begin{figure}[ht]
\centering
\includegraphics[scale = .2]{Figures/taxonomy_distribution.jpg}
\caption{Each individual image in a batch has its own set of hard negatives. This leads to a different target hardness distribution for each image.}
\label{fig: batch_view}
\end{figure}


To integrate hardness within contrastive learning, we must first estimate the target hardness distribution. This distribution represents the effective weighting that should be assigned to each negative sample based on its level of semantic similarity with the anchor image. Ideally, true hard negatives should have a high peak with low variance to represent the relative importance of the hard negative set compared to all other instances in the batch. For example, the anchor image of a flamingo  in Figure \ref{fig: batch_view} is associated with a target hardness distribution with a peak at the negative associated with its most similar sample (the spoonbill) and a lower weighting associated with the other samples in the batch. However, the main challenge with integrating hardness in contrastive learning is that the target hardness distribution is not trivial to estimate in an unsupervised manner. Previous work \cite{robinson2020contrastive} attempted to imbue hardness by constructing an ideal hardness distribution and then approximating it using Monte-Carlo (MC) importance sampling on the data distribution. By performing sampling in this manner, the resultant distribution is meant to assign weights on negatives that reflect the discussed hardness structure. However, the main limitation of their methodology is that the quality of an importance sampling approximation is tied directly to how similar the target and sampling distributions are to each other \cite{tokdar2010importance}. In the case of the target hardness distribution, a quality approximation isn't guaranteed with their method because the sampling distribution is fixed as the data distribution while the target distribution constantly changes depending on the current anchor image of interest. For example, we see in Figure \ref{fig: batch_view} that the set of hard and regular negatives as well as the target hardness distribution is different for each instance in the batch. Thus, previous hardness integration attempts are noisy estimates because they compute the hardness distribution with respect to the entire batch of negatives, rather than adapting its sampling in a customized manner to each anchor.  

In order to achieve a better approximation of the hardness distribution at a per-image level, we propose a framework called adaptive contrastive learning (ACL). Within this framework, we reimagine the hardness approximation process through the lens of multiple MC importance sampling \cite{veach1995optimally}. The idea here is  to perform sampling on a weighted combination of components of the overall distribution, instead of sampling from the entire data distribution as a whole. To further reflect our hardness setting, we also condition that component distributions are computed as a function of individual anchor images to account for the varying hardness distributions shown in Figure \ref{fig: batch_view}. To do this in an unsupervised manner, we introduce a decomposition methodology that divides the set of negatives into a hard and regular subset based on thresholding pairwise cosine similarity values of each negative instance with the current anchor image.  We then approximate the hardness distribution using MC importance sampling on only the hard negative subset and then train with the resultant adaptive contrastive loss. Additionally, from an application point of view, many domains have a structure to their data that readily allows the identification of hard examples. Information such as clinical data within the medical domain \cite{kokilepersaud2022clinical}, noise characteristics in distorted settings \cite{kokilepersaud2023exploiting,kokilepersaud2022volumetric}, and object taxonomy hierarchies \cite{krizhevsky2009learning} all form superclasses that can be exploited as hard negatives. We observe this in Figure \ref{fig: batch_view} where images that are members of the same taxonomy (birds and fish) are hard negatives. However, existing methods do not provide a mechanism by which to explicitly make use of these accessible hardness distributions. We also explore how the general structure of our ACL framework lends itself easily to these other settings.  
In summary, we make the following contributions:
\begin{enumerate}
    \item We propose a new methodology to approximate semantic hardness within the representation space called adaptive contrastive learning.
    \item We present theory related to the connection of our method with   
 MC multiple importance sampling and empirically validate the approximation improvement.
    \item We demonstrate the utility of the proposed ACL in unsupervised, semi-supervised, and supervised setups by either estimating the decomposition through cosine similarity or making use of explicit label information while incurring negligible additional computational cost. 
    \item We demonstrate that our approach outperforms state of the art contrastive learning algorithms in optimal training settings as well as across a wide variety of datasets. 
    
\end{enumerate}

==> Sections/methodology.tex <==
\section{Methodology}

In our TaxCL framework, our goal is to decompose the set of all negatives from $\sum_{a\in{A(i)}}exp(z_{i}\cdot z_{a}/\tau)$ to $\sum_{a\in{A(i)}}exp(z_{i}\cdot z_{a}/\tau)  = \sum_{t\in{T(i)}}exp(z_{i}\cdot z_{d}/\tau) + \sum_{n\notin{T(i)}}exp(z_{i}\cdot z_{n}/\tau) $ where $T(i)$ is a subset of $A(i)$ that represents the taxonomic negatives in the batch. We consider an unsupervised and semi-supervised setting for this loss function. Within the unsupervised setting, we compute the dot product between the positive embedding $z_{i}$ and each negative embedding $z_{a}$ to produce a dot product set of the form $K = [z_{i} \cdot z_{a1}, ... , z_{i} \cdot z_{a(N-2)} ]$. This vector is normalized between 0 and 1. We then introduce a threshold parameter $\epsilon$ where negative embeddings in $K$ that produce a dot product with $z_{i}$ greater than $\epsilon$ will be included as part of $T(i)$ while elements of K less than $\epsilon$ will be excluded from the set $T(i)$. Negatives that are members of $T(i)$ are referred to as $z_{t}$ while all other negatives have the convention of $z_{n}$. There are then a variety of ways to introduce an additional weighting on the taxonomic negatives.   Similarly to \cite{robinson2020contrastive}, . The overall process for computing our loss is detailed visually in Figure \ref{fig: main_visual}. The associated loss is what we refer to as the unsupervised TaxCL  loss and it has the form: 
\begin{equation}
\small
L_{TaxCL} = -\sum_{i\in{I}} log\frac{exp(z_{i}\cdot z_{j(i)}/\tau)}{ exp(z_{i}\cdot z_{j(i)}/\tau) + Q_{ti}\sum_{t\in{T(i)}}exp(z_{i}\cdot z_{t}/\tau) + \sum_{n\notin{T(i)}}exp(z_{i}\cdot z_{n}/\tau)} 
\label{eq:DD}
\end{equation}


\begin{figure*}[ht]
\centering
\includegraphics[scale = .35]{Figures/methodology.jpg}
\caption{This is the process by which the TaxCL loss is computed in a semi-supervised and unsupervised fashion.}
\label{fig: main_visual}
\end{figure*}

==> Sections/related_work.tex <==
\section{Related Work}

\subsection{Positive and Negative Relationship Manipulation} 

Research within contrastive learning has primarily revolved around the idea of manipulating a defined set of positives and negatives \cite{chen2020simple,dwibedi2021little,chen2020improved,li2020prototypical,khosla2020supervised}. A subset of this work has involved adapting positive selection towards specific application domains such as medicine\cite{kokilepersaud2022clinical,kokilepersaud2022gradient}, fisheye object detection, \cite{kokilepersaud2023exploiting}, and associating seismic structures \cite{kokilepersaud2022volumetric}. More general work has included ideas such as removing the influence of false negatives \cite{huynh2022boosting}, developing robust weightings of positive and negative sets  \cite{chuang2022robust}, and creating new types of representations \cite{lavoie2022simplicial}. There is also a subset of works that revolve around the concept of exploiting the relationship between the positive set and the negative set. This includes introducing a term to decouple positive and negative samples \cite{yeh2022decoupled}, performing distance regularization \cite{chen2021large}, selecting negative samples based on a ring of distances from the anchor point \cite{wu2020conditional}, creating mixtures of the batch \cite{shen2022mix}, and making use of inter-anchor relationships \cite{zhang2022dual}. While these works are similar to ours in the sense of exploiting positive and negative relationships, instead of categorizing data into positives and negatives, we categorically view data as part of a spectrum of hardness.
\subsection{Hierarchies and Taxonomies in Contrastive Learning} 

==> Sections/results_analysis.tex <==
\section{Results Analysis}
\subsection{Training Setup}
\subsection{Decomposition Analysis}
\input{Tables/dataset_comparison}

\input{Tables/decomposition_ablation}

\input{Tables/sota_comparison}
